OmniSat: Self-Supervised Modality Fusion for Earth Observation

The diversity and complementarity of sensors available for Earth Observations (EO) calls for developing bespoke self-supervised multimodal learning approaches. However, current multimodal EO datasets and models typically focus on a single data type, either mono-date images or time series, which limits their impact. To address this issue, we introduce OmniSat, a novel architecture able to merge diverse EO modalities into expressive features without labels by exploiting their alignment. To demonstrate the advantages of our approach, we create two new multimodal datasets by augmenting existing ones with new modalities. As demonstrated for three downstream tasks -- forestry, land cover classification, and crop mapping -- OmniSat can learn rich representations without supervision, leading to state-of-the-art performances in semi- and fully supervised settings. Furthermore, our multimodal pretraining scheme improves performance even when only one modality is available for inference. The code and dataset are available at https://github.com/gastruc/OmniSat.

==> 3_method_bk.tex <==
%auto-ignore

We consider a multimodal dataset $x$, defined as a collection of tiles divided into a set $\bP$ of $P$ small spatial patches. We denote by $\bM$ the set of $M$ available modalities.
The patches are defined consistently across modalities: 
$x^\bM_p=\{x^m_p\}_{m\in \bM}$
corresponds to $M$ distinct views of the same patch $p$ with different sensors or modalities. Each modality $m$ has its unique input space $\Omega^m$ such that $x^m_p \in \Omega^m$.
We define an input token as a pair $(m,p)$ for a given modality $m$ and a patch $p$, for a total of $M\times P$ tokens. 

Our goal is to learn multimodal representations $f^\star_p$ that capture the content of each spatial patch $p$ captured by all modalities $\bM$ in a self-supervised fashion. To achieve this, we employ a cross-modal contrastive objective (\secref{sec:contrast}) and a multimodal masked encoding task (\secref{sec:mae}). We then give further details on the implementation of each module in \secref{sec:implem}. The overall architecture is represented in \figref{fig:pipeline}.
%

%--------------------------------------------------------------------
\subsection{Contrastive Objective}
%--------------------------------------------------------------------
\label{sec:contrast}
We associate each modality $m$ with a dedicated patch encoder $\Enc^m: \Omega^m \mapsto \mathbf{R}^d$ and denote by $f^m_p = \Enc^m(x^m_p)$ the $d$-dimensional embedding of the input token $x^m_p$.
We would like $f^m_p$ to capture robust and expressive features of $x^m_p$. To do so, we build a matching objective: patches should have consistent embeddings \emph{across modalities}. Indeed, while each modality captures distinct characteristics of $p$, all encodings $f^m_p$ share the same latent variable: the semantic content of patch $p$.


In practice, we want $f^m_p$ close to $f^n_p$ for $n\neq m$, but far from $f^n_q$ for other patches $q\neq p$.  
We adapt the classic InfoNCE loss  \cite{oord2018representation} to our setting with two main differences, illustrated in \figref{fig:contrast}:
(i) each token $(m,p)$ has $M-1$ positive matches: the tokens corresponding to the same patch $p$ but viewed in another modality $n\neq m$; %, similar to the multi-positive contrastive loss MIL-NCE ;
and (ii) as EO observations are generally spatially regular, nearby patches may be visually indistinguishable. Therefore, we exclude from the negative matches of $(m,p)$ all tokens in modality $m$ that are too close to $p$. To this end, we remove the set $T(m,p)$ of tokens with modality $m$ and whose patches are in the same tile as $p$.
Our loss function $\Lcon$ is defined as such:
\begin{align}
    \Lcon = \frac1{MP}
    \sum_{(m,p) \in \bM \times \bP}
    \log 
    \left(
        \frac
        {
        \sum_{n \neq m}
            \exp(\langle f^m_p, f^n_p\rangle / \gamma)
        }
        {
        \sum_{(n,q)\in \bM\times \bP \setminus T(m,p)}
            \exp(\langle f^m_p, f^n_q\rangle / \gamma)
        }
    \right)~,
\end{align}
with $\gamma$ a temperature parameter,  and 
$\langle \cdot,\cdot\rangle$ the scalar product in $\bR^d$.
This function, specifically designed for geospatial data, allows us to contrast individual patches across modalities, which is not typically feasible for natural images.
%
However, as the contrastive objective aligns multimodal representations, the patch encoders $\cE^\bM$ may be encouraged to overlook the distinct attributes of their respective modality. Instead, they may focus only on features shared by all modalities, \ie their \emph{common denominator}. To ensure that encoders also capture modality-specific information, we incorporate a reconstruction objective, detailed in \secref{sec:mae}.

 \begin{figure}[t]
     \centering
     \begin{minipage}[c]{0.6\textwidth}
    \input{figures/contrast_eccv}
    \end{minipage}
    \hfill
    \begin{tabular}{c}
    \begin{minipage}[c]{0.35\textwidth}
    \caption{{\bf Contrastive Loss.} We represent the token matching matrix for two tiles $T_1$ and $T_2$  viewed across $3$ modalities $m_1$, $m_2$, and $m_3$. $T_1$ is composed of the patches $p_1$ and $p_2$, while $T_2$ comprises $q_1$ and $q_2$. In contrast to classic approaches which ignore the diagonal and assign each sample with a single positive match, our loss defines operates at the patch level, considers multiple positives per token, and excludes tokens in a block-diagonal fashion.
    }
    \label{fig:contrast}
    \end{minipage}
    \\
     \begin{minipage}[c]{0.35\textwidth}
    \centering 
    \begin{tabular}{r@{\;\;}l}
    \tikz[baseline]  \node [fill=green, minimum width=4mm, minimum height=4mm,anchor=base] {+};&\small positive match
    \\
   \tikz[baseline]  \node [fill=red!50, minimum width=4mm, minimum height=4mm,anchor=base] {-\vphantom{+}};&\small negative match
   \\
   \tikz[baseline]  \node [fill=black!30, minimum width=4mm, minimum height=4mm,anchor=base] {o\vphantom{+}};&\small ignored
    \end{tabular}
    \end{minipage}
    \end{tabular}
 \end{figure}

%---------------------------------------------------------------------
\subsection{Multimodal Reconstruction Objective}
%---------------------------------------------------------------------
\label{sec:mae}
This section introduces the modality combiner network $\comb$ and its reconstruction objective.
We mask a fraction of tokens $\mask \subset \bM\times \bP$ and replace their embeddings with a learned vector $f^\text{mask} \in \bR^d$. Note that the masking can differ across modalities, and some patches may be entirely masked.
All tokens are then processed by the modality combining network $\comb$, which outputs $P$ multimodal embeddings $f^\star_{\bP}$:
\begin{align}
    f_\bP^\star= \comb
    \left(
    \{f^m_p\}_{(m,p) \not\in \mask}
    \cup
    \{f^\text{mask}\}_{(m,p) \in \mask}
    \right)~.
\end{align}
To encourage the patch embeddings $f^\star_{\bP}$ to capture information from all modalities, we build a multimodal reconstruction objective.
We equip each modality $m$ with a dedicated decoder $\Dec^m:\bR^d \mapsto \Omega^m$ and write the reconstruction loss as:
\begin{align}
    \Lmae =
    \frac1{\vert \mask \vert}
    \sum_{(m,p) \in \mask} 
    \frac1{\text{dim}(\Omega^m)}
    \left\Vert 
        \Dec^m(f^\star_p) - x^m_p
    \right\Vert^2~,
\end{align}
where $\text{dim}(\Omega^m)$ is the dimension of the input space $\Omega^m$.
The total loss is the sum of $\Lmae$ and $\Lcon$.% weighted by a factor $\lambda_\text{contrast}=1$.

%==========================================
\subsection{Implementation }
%==========================================
\label{sec:implem}
This section presents the tokenization process, the structure of the encoder and decoder for each modality, and the architecture of the modality combiner network. In particular, we highlight several design choices that leverage the specific properties of EO data \cite{rolf2024mission}.

\parag{\bf Multimodal Tokenization.}
All available modalities are spatially aligned through georeferencing. We split each tile along a regular spatial grid to produce a set of non-overlapping patches $\bP$ consistent across all modalities, thus ensuring that $x^\bM_p$ correspond to the same area for all modalities. 

{For TreeSat and FLAIR, we use a $10\times10$m grid, meaning that the VHR input tokens are small image patches of size $50\times 50$ with $0.2$m per pixel. The patches of Sentinel observations with a resolution of $10$m are single-pixel temporal sequences of spectral measurements. For PASTIS-HD, we use a $40\times40$m grid, meaning that the VHR patches are of size $40\times 40$ with $1.0$m per pixel. The patches of Sentinel observations \cite{Sentinel-2-paper} are $4\times4$ image time series which we spatially flatten before encoding.}

%Throughout all experiments, we use a grid with cells of $10\times10$m, but this value could be adapted to other applications. A patch from a VHR observation is a small image patch of size $50\times 50$ with $0.2$m per pixel, or $1\times1$ at $10$m resolution. The patches of Sentinel observations \cite{Sentinel-2-paper}, which have a resolution of $10$m, are single-pixel temporal sequences of spectral measurements.

Time series from Sentinel satellites may experience registration errors spanning several meters, complicating their precise alignment with high-resolution imagery. However, using temporal sequences of satellite data mitigates these errors as aggregation over time tends to balance out misalignments.

\parag{\bf Encoder-Decoder for Images.}
Image tiles are split into small square patches: $\Omega^\text{img}=\bR^{C \times I \times I}$ with $I$ the size of the patches and $C$ the number of channels. As shown in \figref{fig:implem:a}, we encode these inputs with a sequence of convolutions and max-pool layers until the spatial dimension is fully collapsed. Decoding involves a symmetric sequence of convolutions and un-pooling layers. Contrary to existing masked auto-encoders, we pass the pooling indices from the encoder's max-pooling to the decoder's un-pooling in the manner of SegNet~\cite{badrinarayanan2017segnet}. This dispenses the encoder from learning the intra-token spatial configuration and allows it to focus on the radiometric information, which may be more relevant depending on the application.
%Single-pixel image tokens are encoded with a Multi-Layer Perceptron (MLP).

\begin{figure*}[t]
    \centering
    \input{figures/implem}
    \caption{{\bf Module's Architectures.} (\subref{fig:implem:a}) represents the encoder and decoder of image patches, and (\subref{fig:implem:b}) illustrates their architectures for temporal patches with a length of $L=4$ time stamps. The modality combining module $\comb$ is depicted in (\subref{fig:implem:c}) with $P=2$ and $M=3$. {Elements colored in {orange} are learned networks or parameters.}}
    \label{fig:enter-label}
\end{figure*}

\parag{\bf Encoder-Decoder for Time Series.}
Each temporal patch is represented by $L$ sequential observations with $C$ channels:  $\Omega^\text{TS}=\bR^{C \times L}$, each associated with a time stamp.
We encode the temporal patches using a Lightweight Temporal Attention Encoder (LTAE) model  \cite{garnot2020lightweight}, an efficient network for geospatial time series processing. We decode each multimodal embedding $f^\star_p$ into temporal patches by repeating it $L$ times across the temporal dimension, adding a temporal encoding for each time step, and using an MLP to map the results to size $C$. See \figref{fig:implem:b} for an illustration.

Optical time series are notoriously affected by clouds \cite{sudmanns2019assessing}. This may affect the validity of the reconstruction task: the decoder cannot know which observations are cloudy, making the reconstruction objective unpredictable. To circumvent this issue, we use the temporal attention maps of the encoder's LTAE to select dates to reconstruct: cloudless observations are more informative and should have a higher attention score \cite{russwurm2020self}. We only consider in the reconstruction loss $\Lmae$ the top $25\%$ dates in terms of the LTAE's attention maps.

\parag{\bf Modality Combining Network.} 
The modality combining network $\comb$, represented in \figref{fig:implem:c}, takes the $M \times P$ token embeddings ${f}^\bM_\bP$, some of whom can potentially be masked. 
We equip each token with a Euclidean relative positional encoding \cite{wu2021rethinking}  calculated based on their patch's position $\{r(p,q) \mid (p,q)\in \bP^2\}$, and only defined for patches within the same tile. This way, each token can selectively consider its spatial surroundings. As most EO data are captured from above (satellite or aerial), their distribution is invariant by horizontal translation, making this choice of encoding preferable to an absolute position encoding.

The modality combining module $\comb$ starts with a series of $B$ residual self-attention blocks connecting all tokens across modality and within the same tile. We then perform cross-attention between the resulting token embeddings $g^\bM_\bP \in \bR^{d \times M \times P}$ and $P$ copies $f^\text{comb}_\bP$ of a modality combining token $f^\text{comb} \in \bR^d$ learned as a free parameter. Each copy of $f^\text{comb}_p$ is spatially located at the patch $p$ for the relative positional encoding $r$. The mechanism of $\comb$ writes:
\begin{align}
    g^\bM_\bP & = \text{self-attention}
    \left(
    {f}^{\bM}_{\bP}; r\right)~, \\
    {f}^\star_\bP & =  \text{cross-attention}
    \left(f^\text{comb}_\bP, g^\bM_\bP ;r
    \right)~.
\end{align}

\parag{\bf Hyperparameters.} To show the versatility of OmniSat, we use the same configuration throughout all experiments. The embedding size is $d=256$, resulting in image encoders and decoders with $3.6$M and $1.8$M parameters, $403$K and $96$K for optical time series, and $402$K and $95$K for radar time series. The modality combiner module is composed of $B=6$ residual self-attention blocks and a single cross-attention block, for a total of $3.6$M parameters. We train our model with the ADAM optimizer \cite{kingma2014adam}, with a learning rate of $10^{-4}$ for pretraining and $2\times 10^{-5}$ for fine-tuning, and a ReduceLROnPlateau scheduler \cite{reduce} with a patience of $10$ epochs and a decay rate of $0.1$. When re-implementing competing methods, we use the hyperparameters of their open-source repository.

%We Split the image into 16 sub images for PASTIS-R due to memory issues

==> figures/contrast.tex <==
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}

\resizebox{\linewidth}{!}{
\begin{tabular}{l@{}l@{}l@{} C{1.2mm}C{1.2mm} C{1.2mm}C{1.2mm} C{1.2mm}C{1.2mm}  C{1.2mm}C{1.2mm} C{1.2mm}C{1.2mm} C{1.2mm}C{1.2mm}}
&&&\multicolumn{6}{c}{$T_1$} & \multicolumn{6}{c}{$T_2$} \\
\cmidrule(r{4pt}){4-9}\cmidrule(r{4pt}){10-15}
&&&\multicolumn{2}{c}{$m_1$}  & \multicolumn{2}{c}{$m_2$} & \multicolumn{2}{c}{$m_3$}
&\multicolumn{2}{c}{$m_1$}  & \multicolumn{2}{c}{$m_2$} & \multicolumn{2}{c}{$m_3$} \\
\cmidrule(r{4pt}){4-5}\cmidrule(r{4pt}){6-7}
\cmidrule(r{4pt}){8-9}\cmidrule(r{4pt}){10-11}
\cmidrule(r{4pt}){12-13}\cmidrule(r{4pt}){14-15} 
&&&$p_1$ & $p_2$ & $p_1$ & $p_2$ & $p_1$ & $p_2$ & $q_1$ & $q_2$ & $q_1$ & $q_2$ & $q_1$ & $q_2$ \\
\multirow{6}{*}{\raisebox{+.8cm}{$T_1$} {\vrule height 2cm}}&\multirow{2}{*}{\raisebox{+.2cm}{$m_1$} \vrule height .6cm} & \vphantom{\vrule height .35cm}$p_1$ &
\cellcolor{black!30}$\mkern-1.5mu$o& \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- \\ 
&& \vphantom{\vrule height .35cm}$p_2$&
\cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- \\
&\multirow{2}{*}{\raisebox{+.2cm}{$m_2$} \vrule height .6cm} & \vphantom{\vrule height .35cm}$p_1$ &
\cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- \\
& & \vphantom{\vrule height .35cm}$p_2$&
\cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- \\
&\multirow{2}{*}{\raisebox{+.2cm}{$m_3$} \vrule height .6cm} & \vphantom{\vrule height .35cm}$p_1$&
\cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- \\
& & \vphantom{\vrule height .35cm}$p_2$&
\cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- \\
\multirow{6}{*}{\raisebox{+.8cm}{$T_2$} {\vrule height 2cm}}&\multirow{2}{*}{\raisebox{+.2cm}{$m_1$} \vrule height .6cm}&\vphantom{\vrule height .35cm}$q_1$ &
 \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50} -\\ 
&& \vphantom{\vrule height .35cm}$q_2$&
 \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ \\
&\multirow{2}{*}{\raisebox{+.2cm}{$m_2$} \vrule height .6cm} & \vphantom{\vrule height .35cm}$q_1$&
 \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- &  \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- \\
& & \vphantom{\vrule height .35cm}$q_2$&
 \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ \\
&\multirow{2}{*}{\raisebox{+.2cm}{$m_3$} \vrule height .6cm} & \vphantom{\vrule height .35cm}$q_1$&
 \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o\\
& & \vphantom{\vrule height .35cm}$q_2$&
 \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{red!50}- & \cellcolor{green}$\mkern-1.5mu$+ & \cellcolor{black!30}$\mkern-1.5mu$o & \cellcolor{black!30}$\mkern-1.5mu$o\\
\end{tabular}
}

==> figures/datasets.tex <==
\centering
\begin{tabular}{cc}
    \begin{subfigure}{0.45\textwidth}
        \centering
        \begin{tabular}{cc}
          \includegraphics[width=.65\linewidth]{images/datasets/Aerial_FLAIR.png} 
          &
          %\vspace{-15mm} 
          \begin{minipage}[t][.05\linewidth][t]{.15\linewidth}
          \vspace{-35mm}
        \begin{tabular}{@{\hspace{0mm}}c}
            \includegraphics[width=.95\linewidth]{images/datasets/S2_FLAIR_30.png}\\
            \includegraphics[width=.95\linewidth]{images/datasets/S2_FLAIR_1.png}\\
            \includegraphics[width=.95\linewidth]{images/datasets/S2_FLAIR_5.png}\\
            \includegraphics[width=.95\linewidth]{images/datasets/S2_FLAIR_15.png}
         \end{tabular}\end{minipage}\\
        \scriptsize  \centering Very high resolution &\scriptsize Sentinel-2\\
       \scriptsize  \centering RGB + NIR + nDSM & \scriptsize time series  \\
        \end{tabular}
        \captionsetup{font=small,labelfont=small}
        \caption{Flair}
         \label{fig:data:flair}
    \end{subfigure}
    \begin{subfigure}{0.55\textwidth}
     \begin{tabular}{ccc}
        \begin{minipage}[t][.05\linewidth][t]{.53\linewidth}
        \vspace{-34.5mm}
        \includegraphics[width=1\linewidth, angle=180]{images/datasets/forest_rgb2.png} 
        \end{minipage}
        &%\vspace{-15mm}
          \begin{minipage}[t][.05\linewidth][t]{.15\linewidth}
          \vspace{-34.5mm}
        \begin{tabular}{@{\hspace{1mm}}c}
        \includegraphics[width=.71\linewidth]{images/datasets/s2-4.png}
        \\
        \contour{black}{$\downarrow$}
        \\
       \includegraphics[width=.71\linewidth]{images/datasets/s2-6.png}
       \\
       \includegraphics[width=.71\linewidth]{images/datasets/s2-3.png}
       \\
       \includegraphics[width=.71\linewidth]{images/datasets/s2-2.png}
        \end{tabular}\end{minipage}
     &%\vspace{-15mm} 
       \begin{minipage}[t][.05\linewidth][t]{.15\linewidth}
       %\vspace{-35mm}
       \vspace{-34.5mm}
        \begin{tabular}{@{\hspace{1mm}}c}
        \includegraphics[width=.71\linewidth]{images/datasets/S1_mono_TSAI.png}
        \\
        \contour{black}{$\downarrow$}
        \\
       \includegraphics[width=.71\linewidth]{images/datasets/S1_TSAI_1.png}
       \\
       \includegraphics[width=.71\linewidth]{images/datasets/S1_TSAI_15.png}
       \\
       \includegraphics[width=.71\linewidth]{images/datasets/S1_TSAI_20.png}
     \end{tabular}\end{minipage}
     \\
       \scriptsize  \centering Very high resolution &  \scriptsize  \bf \centering $\star$ Sentinel-2 & \scriptsize \bf $\star$  Sentinel-1\\
      \scriptsize \centering  RGB + NIR &  \scriptsize \bf time series   & \scriptsize \bf \;\;  time series    \\
     \end{tabular}
     \captionsetup{font=small,labelfont=small}
        \caption{TreeSatAI-TS}
         \label{fig:data:treesat}
    \end{subfigure}
\end{tabular}

\if 10
\centering
\begin{tabular}{cc}
    \begin{subfigure}{0.45\textwidth}
        \centering
        \begin{tabular}{m{.65\textwidth}m{.33\textwidth}}
          \includegraphics[width=1\linewidth]{images/datasets/Aerial_FLAIR.png} 
          &
          \vspace{-15mm} 
        \begin{tabular}{@{\hspace{3mm}}c}
            \includegraphics[width=.44\linewidth]{images/datasets/S2_FLAIR_30.png}\\
            \includegraphics[width=.44\linewidth]{images/datasets/S2_FLAIR_1.png}\\
            \includegraphics[width=.44\linewidth]{images/datasets/S2_FLAIR_5.png}\\
            \includegraphics[width=.44\linewidth]{images/datasets/S2_FLAIR_15.png}
         \end{tabular}\\
        \scriptsize  \centering Very high resolution &\scriptsize Sentinel-2\\
       \scriptsize  \centering RGB + NIR + nDSM & \scriptsize time series  \\
        \end{tabular}
        \caption{Flair}
         \label{fig:data:flair}
    \end{subfigure}
    \begin{subfigure}{0.55\textwidth}
     \begin{tabular}{m{.53\textwidth}m{.23\textwidth}m{.23\textwidth}}
        \includegraphics[width=1\linewidth]{images/datasets/forest_rgb2.png} 
        &\vspace{-15mm}
        \begin{tabular}{@{\hspace{3mm}}c}
        \includegraphics[width=.45\linewidth]{images/datasets/s2-4.png}
        \\
        \contour{black}{$\downarrow$}
        \\
       \includegraphics[width=.45\linewidth]{images/datasets/s2-6.png}
       \\
       \includegraphics[width=.45\linewidth]{images/datasets/s2-3.png}
       \\
       \includegraphics[width=.45\linewidth]{images/datasets/s2-2.png}
        \end{tabular}
     &\vspace{-15mm} 
        \begin{tabular}{@{\hspace{3mm}}c}
        \includegraphics[width=.45\linewidth]{images/datasets/S1_mono_TSAI.png}
        \\
        \contour{black}{$\downarrow$}
        \\
       \includegraphics[width=.45\linewidth]{images/datasets/S1_TSAI_1.png}
       \\
       \includegraphics[width=.45\linewidth]{images/datasets/S1_TSAI_15.png}
       \\
       \includegraphics[width=.45\linewidth]{images/datasets/S1_TSAI_20.png}
     \end{tabular}
     \\
       \scriptsize  \centering Very high resolution &  \scriptsize  \bf \centering $\star$ Sentinel-2 & \scriptsize \bf $\star$  Sentinel-1\\
      \scriptsize \centering  RGB + NIR &  \scriptsize \bf \quad time series   & \scriptsize \bf \;\;  time series    \\
     \end{tabular}
        \caption{TreeSatAI-TS}
         \label{fig:data:treesat}
    \end{subfigure}
\end{tabular}*
\fi

==> figures/datasets_pastis_poster.tex <==
\begin{tabular}{ccc}
        \begin{minipage}[t][.2\textheight][t]{.3\linewidth}
        \centering
        \begin{tabular}{c}
         \scriptsize VHR  \\
        \includegraphics[width=.76\linewidth]{images/datasets/Aerial_FLAIR.png}
        \\
        \scriptsize Sentinel-2 time series
         \\
         \begin{tabular}{cc}
            \includegraphics[width=.28\linewidth]{images/datasets/S2_FLAIR_30.png}&
            \includegraphics[width=.28\linewidth]{images/datasets/S2_FLAIR_1.png}\\
            \includegraphics[width=.28\linewidth]{images/datasets/S2_FLAIR_5.png}&
            \includegraphics[width=.28\linewidth]{images/datasets/S2_FLAIR_15.png}
         \end{tabular}
        \end{tabular}
        \end{minipage}
          %\caption{FLAIR}
    &
    \begin{minipage}[t][.2\textheight][t]{.3\linewidth}
        \centering
        \begin{tabular}{m{.2\linewidth}@{\,}m{.1\linewidth}@{\,}m{.2\linewidth}@{\,}m{.2\linewidth}@{\,}m{.2\linewidth}}
        \multicolumn{5}{c}{\scriptsize VHR RGB+NIR}        \vspace{-2.8mm}
        \\
        \multicolumn{5}{c}{\includegraphics[angle=180,width=.8\linewidth]{images/datasets/forest_rgb2.png}}
        \vspace{1mm}
        \\
        \multicolumn{5}{c}{\scriptsize \large{$\star$}\scriptsize~Sentinel-2 \bf{time series} }\\
        \includegraphics[width=1\linewidth, height=.025\textheight]{images/datasets/s2-4.png}
        &
        \contour{black}{$\rightarrow$}
        &
       \includegraphics[width=1\linewidth, height=.025\textheight]{images/datasets/s2-6.png}
       &
       \includegraphics[width=1\linewidth, height=.025\textheight]{images/datasets/s2-3.png}
       &
       \includegraphics[width=1\linewidth, height=.025\textheight]{images/datasets/s2-2.png}
       \\
       \multicolumn{5}{c}{\scriptsize {\large{$\star$}\scriptsize}~Sentinel-1 \bf{time series}}
       \\
        \includegraphics[width=1\linewidth, height=.025\textheight]{images/datasets/S1_mono_TSAI.png}
        &
        \contour{black}{$\rightarrow$}
        &
       \includegraphics[width=1\linewidth, height=.025\textheight]{images/datasets/S1_TSAI_1.png}
       &
       \includegraphics[width=1\linewidth, height=.025\textheight]{images/datasets/S1_TSAI_15.png}
       &
       \includegraphics[width=1\linewidth, height=.025\textheight]{images/datasets/S1_TSAI_20.png}
        \end{tabular}
        \end{minipage}
        %\caption{\bf TreeSatAI-TS}
    &
        \begin{minipage}[t][.2\textheight][t]{.3\linewidth}
        \centering
         \begin{tabular}{c}
        \scriptsize PASTIS: Sentinel-2 TS
        \\
        \begin{tabular}{c@{\,}c@{\,}c@{\,}c}
        \includegraphics[width=.22\linewidth, height=.025\textheight]{images/datasets/S2_pastis_5.png}&        \includegraphics[width=.22\linewidth, height=.025\textheight]{images/datasets/S2_pastis_15.png} &       \includegraphics[width=.22\linewidth, height=.025\textheight]{images/datasets/S2_pastis_25.png} &       \includegraphics[width=.22\linewidth, height=.025\textheight]{images/datasets/S2_pastis_30.png}
        \end{tabular}
        \\
        \scriptsize{PASTIS-R: + Sentinel-1 TS}
        \\
         \begin{tabular}{c@{\,}c@{\,}c@{\,}c}   
        \includegraphics[width=.22\linewidth, height=.025\textheight]{images/datasets/S1_pastis_10.png}
        &
        \includegraphics[width=.22\linewidth, height=.025\textheight]{images/datasets/S1_pastis_15.png}
        &
        \includegraphics[width=.22\linewidth, height=.025\textheight]{images/datasets/S1_pastis_25.png}
        &
        \includegraphics[width=.22\linewidth, height=.025\textheight]{images/datasets/S1_pastis_40.png}
          \end{tabular}
        \\
        \scriptsize \scriptsize{\large{$\star$}\scriptsize} \bf{VHR RGB} 
         \\
        \includegraphics[width=.8\linewidth]{images/datasets/spot_pastis.png}
        \end{tabular}
        \end{minipage}
        %\caption{\bf PASTIS-HD}
        \\
        FLAIR & TreeSatAI-TS & PASTIS
    \end{tabular}

==> figures/failure.tex <==
\begin{tabular}{l ll l lll}
    &\multicolumn{2}{c}{\scriptsize  Inputs} & \scriptsize Ground truth & \bf \scriptsize \underline{OmniSat} &  \scriptsize UT\&T \cite{garioud2023flair} & \scriptsize Scale-\scriptsize MAE \cite{reed2023scale} \\
    \rotatebox{90}{\;\;\;\;\scriptsize  TreeSatAI-TS}
     &
      \includegraphics[width=.17\linewidth, angle=180,origin=c]{images/fail_tree_vhr.png}
    &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-23.5mm}\centering
    \begin{tabular}{c@{\;}c}
        \includegraphics[width=.38\linewidth]{images/fail_tree_s21.png}
        &
        \includegraphics[width=.38\linewidth]{images/fail_tree_s11.png}
       \\
       \includegraphics[width=.38\linewidth]{images/fail_tree_s24.png}
       &
    \includegraphics[width=.38\linewidth]{images/fail_tree_s12.png}
       \\
       \includegraphics[width=.38\linewidth]{images/fail_tree_s25.png}
       &
    \includegraphics[width=.38\linewidth]{images/fail_tree_s13.png}
    \end{tabular}
    \end{minipage}
     &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-21mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
        - Quercus \tiny \faLeaf\\
        - Acer \tiny \faLeaf\\
        - Alnus \tiny \faLeaf\\
        - Larix \tiny \faTree\\
        
     \end{tabular}}
      \end{minipage}
          &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-21mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
        - \textcolor{green!50!black}{Quercus}  \\
        - \textcolor{red!50!black}{\xmark} \\
        - \textcolor{red!50!black}{\xmark}\\
        - \textcolor{red!50!black}{\xmark} \\
        - \textcolor{red!50!black}{Abies} \tiny \faTree \\

     \end{tabular}}
      \end{minipage}
      &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-21mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{\xmark} \\
         - \textcolor{red!50!black}{Abies} \tiny \faTree \\
         - \textcolor{red!50!black}{Betula}  \tiny \faLeaf
     \end{tabular}}
      \end{minipage}
     &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-21mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - \textcolor{red!50!black}{\xmark} \\
         - \textcolor{red!50!black}{\xmark} \\
         - \textcolor{red!50!black}{\xmark} \\
         - \textcolor{red!50!black}{\xmark} \\
         - \textcolor{red!50!black}{Picea} \tiny \faTree\\
     \end{tabular}}
      \end{minipage}
     \\~\\~\\
    \rotatebox{90}{\;\qquad\scriptsize  FLAIR}
     &
      \includegraphics[width=.17\linewidth, angle=0]{images/fail_aerial_FLAIR.png}
    &
     \begin{minipage}[t][.10\linewidth][t]{.13\linewidth}
     \vspace{-23.5mm}\centering
    \begin{tabular}{@{\;}c}
        \includegraphics[width=.38\linewidth,angle=0, origin=c]{images/fail_flair_s21.png}
       \\
       \includegraphics[width=.38\linewidth,angle=0, origin=c]{images/fail_flair_s22.png}
       \\
    \includegraphics[width=.38\linewidth,angle=0, origin=c]{images/fail_flair_s23.png}
    \end{tabular}
    \end{minipage}
     &
     \begin{minipage}[t][.10\linewidth][t]{.13\linewidth}
     \vspace{-23.5mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - decideous \\
         - herbaceous\\
         - water \\
         - pervious surf.\\
         - bare soil
     \end{tabular}}
      \end{minipage}
          &
     \begin{minipage}[t][.10\linewidth][t]{.13\linewidth}
     \vspace{-23.5mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - \textcolor{green!50!black}{decideous}\\
         - \textcolor{green!50!black}{herbaceous}\\
         - \textcolor{green!50!black}{water}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{building}\\
         - \textcolor{red!50!black}{imperv. surf.}\\
         - \textcolor{red!50!black}{brushwood}
     \end{tabular}}
      \end{minipage}
         &
     \begin{minipage}[t][.10\linewidth][t]{.13\linewidth}
     \vspace{-23.5mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - \textcolor{green!50!black}{decideous}\\
         - \textcolor{green!50!black}{herbaceous}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{green!50!black}{pervious surf.}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{building}\\
         - \textcolor{red!50!black}{imperv. surf.}\\
         - \textcolor{red!50!black}{brushwood}\\
         - \textcolor{red!50!black}{coniferous}
     \end{tabular}}
      \end{minipage} 
          &
     \begin{minipage}[t][.10\linewidth][t]{.13\linewidth}
     \vspace{-23.5mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - \textcolor{green!50!black}{decideous}\\
         - \textcolor{green!50!black}{herbaceous}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{green!50!black}{pervious surf.}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{building}\\
         - \textcolor{red!50!black}{imperv. surf.}\\
         - \textcolor{red!50!black}{brushwood}\\
         - \textcolor{red!50!black}{coniferous}\\
         - \textcolor{red!50!black}{other}
     \end{tabular}}
      \end{minipage}
     \\
    \rotatebox{90}{\;\;\;\;\;\;\scriptsize PASTIS-HD}
     &
      \includegraphics[width=.17\linewidth, angle=0]{images/Aerial_PASTIS_failure.png}
    &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-23.5mm}\centering
    \begin{tabular}{c@{\;}c}
        \includegraphics[width=.38\linewidth]{images/pastis_s2f_1.png}
        &
        \includegraphics[width=.38\linewidth]{images/pastis_s1f_1.png}
       \\
       \includegraphics[width=.38\linewidth]{images/pastis_s2f_2.png}
       &
    \includegraphics[width=.38\linewidth]{images/pastis_s1f_2.png}
       \\
       \includegraphics[width=.38\linewidth]{images/pastis_s2f_3.png}
       &
    \includegraphics[width=.38\linewidth]{images/pastis_s1f_3.png}
    \end{tabular}
    \end{minipage}
     &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-23.4mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - Meadow \\
         - Winter wheat \\
         - Corn \\
         - Potatoes \\
         - Mixed cereal
     \end{tabular}}
      \end{minipage}
          &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-23.4mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - \textcolor{green!50!black}{Meadow} \\
         - \textcolor{green!50!black}{Winter wheat} \\
         - \textcolor{green!50!black}{Corn} \\
         - \textcolor{green!50!black}{Potatoes} \\
         - \textcolor{red!50!black}{\xmark} \\
         - \textcolor{red!50!black}{Winter barley}\\
         - \textcolor{red!50!black}{Wint. rapeseed}\\
         - \textcolor{red!50!black}{Legum. fodder}\\
     \end{tabular}}
      \end{minipage}
         &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-23.4mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - \textcolor{green!50!black}{Meadow} \\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{\xmark}\\
         - \textcolor{red!50!black}{Spring barley}\\
         - \textcolor{red!50!black}{Orchard}\\
         - \textcolor{red!50!black}{Legum. fodder}\\
         - \textcolor{red!50!black}{Durum wheat}\\
         - \textcolor{red!50!black}{Fruits, veg..}
     \end{tabular}}
      \end{minipage} 
          &
     \begin{minipage}[t][.01\linewidth][t]{.13\linewidth}
     \vspace{-23.4mm}\scriptsize {
     \begin{tabular}{m{\linewidth}}
         - \textcolor{green!50!black}{Meadow} \\
         - \textcolor{green!50!black}{Winter wheat} \\
         - \textcolor{green!50!black}{Corn} \\
         - \textcolor{red!50!black}{\xmark} \\
         - \textcolor{red!50!black}{\xmark} \\
         - \textcolor{red!50!black}{Winter barley}\\
         - \textcolor{red!50!black}{Wint. rapeseed}\\
         - \textcolor{red!50!black}{Winter triticale}\\
     \end{tabular}}
      \end{minipage}
      ~\\~\\
\end{tabular}

==> suppmat.tex <==
\renewcommand\thefigure{A-\arabic{figure}}
\renewcommand\thesection{A-\arabic{section}}
\renewcommand\thetable{A-\arabic{table}}
\renewcommand\theequation{A-\arabic{equation}}
%\renewcommand\thealgorithm{A-\arabic{algorithm}} 

\input{figures/visualizer}

In this document, we introduce our interactive visualization tool (\secref{sec:visu}), XXXX

%==============================================
\section{Interactive Visualization}
%==============================================
\label{sec:visu}

We release for this project an interactive visualization tool 
{which produces} HTML files compatible with any browser. As shown in 
{\figref{fig:visu},}
we can visualize samples from the datasets with different point attributes and from any angle. These visualizations were instrumental in designing and validating our model, and we hope that they will be help the reader's understanding as well.

%==============================================
\section{Source Code}
%==============================================
\label{sec:code}

% We make our source code available to the reader, along with indications for installing the project and reproducing our main results on S3DIS, KITTI-360, and DALES. 
% This code will be publicly released upon publication.
{
We make our source code publicly available at \GITHUB.
The code provides all necessary instructions for installing and navigating the project, simple commands to reproduce our main results on all datasets, off-the-shelf pretrained models, and ready-to-use notebooks. 
}
Our method is developed in Pytorch and relies on the libraries PyTorch Geometric, PyTorch Lightning, and Hydra. 

%==============================================
\section{Limitations}
%==============================================
\label{sec:limitations}

%==============================================
\section{Implementation Details}
%==============================================
\label{sec:implem}

\subsection{UT&T \cite{garioud2023flair}}

% Pour moi ces info ci dessous vont aller dans le sup mat 
The UNet of UT\&T has a ResNet-34 backbone partially initialized with a RGB ResNet pre-trained on ImageNet but it is not the case for the UTAE branches. 

%In the case of PASTIS-HD, the cloudy images can not be filtered out because this information is not available. 
In the case of TreeSat AI, the aerial image are resized to (as the UNet need a input size multiple of 32). The UTAE branches are reduced to a smaller size due to the small size of the Sentinel images. 
All the model are trained for 100 epochs monitored by an early stoppping with a patience of 30 epochs on the validation loss (of all the modalities). 

%We also average the S1 time series per month on both Pastis-HD and TreeSatAI-TS.

%For Pastis-HD, we Split the image into 8 sub images for PASTIS-R due to memory issues.

%==============================================
\section{Detailed Results}
%==============================================
\label{sec:classwise}

\input{tables/classwise}

We report in \tabref{tab:classwise} the class-wise performance across all datasets for \SHORTHAND and other methods for which this information was available. 

\balance

\input{tables/colormaps}

%==============================================
%==============================================
%\section{Supplementary Visualization}
%==============================================
%extra vizs: failure cases
%only if you have time

==> templates/3DV/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> z_backup_pastis/1_intro.tex <==
Self-supervised learning of multimodal representations has become an area of significant interest within the computer vision community \cite{zong2023self,girdhar2023imagebind,shukor2023unival}. Earth Observation (EO) offers a unique opportunity to apply and advance self-supervised and multimodal approaches, thanks to its wealth of open-access data and diverse sensing technologies with complementary capabilities \cite{ghamisi2019multisource,schmitt2016data}. 
Integrating diverse sources of EO observations to create rich multimodal representations is crucial for several high-impact applications, including environmental \cite{coppin2002digital,secades2014earth,skidmore2021priority} and climate monitoring \cite{yang2013role,lacoste2021toward}, as well as improving food security \cite{nakalembe2020urgent}. Moreover, learning with few or no labels is essential for developing regions with limited data annotation capabilities \cite{kuffer2020role,anderson2017earth,mai2023opportunities}. This work addresses these challenges by proposing a novel self-supervised approach for EO modality fusion.

Currently, most multimodal EO datasets and models focus on a single data type, either mono-date images or time series. This limitation prevents them from simultaneously leveraging the spatial resolution of aerial images \cite{li2012current,manfreda2018use}, the temporal and spectral resolutions of optical satellite time series \cite{Sentinel-2-paper}, and the resilience of radar to weather effects \cite{moreira2013tutorial,amitrano2021earth}. 
Furthermore, existing approaches are often specialized for a given set of sensors, resulting in poor generalization and limited applicability to downstream tasks.

To address these challenges, we propose OmniSat, a novel architecture designed for the self-supervised fusion of diverse multimodal EO data. 
\LOIC{Unlike existing multimodal approaches that map multiple unrelated inputs to a pivot modality \cite{shukor2023unival,girdhar2023imagebind} or a shared latent space \cite{girdhar2022omnivore,srivastava2024omnivec}, OmniSat aims to combine multimodal views of the same area into one unique representation. }
%Unlike existing multimodal approaches that align multiple inputs to a pivot modality \cite{shukor2023unival,girdhar2023imagebind} or a shared latent space \cite{girdhar2022omnivore,srivastava2024omnivec}, OmniSat aims to leverages and combines the unique characteristics of each modality.
OmniSat learns to merge these features into a single representation richer than what could be achieved with each modality individually \cite{recasens2023zorro,greenwell2024watch,benedetti2018m}.

In computer vision, obtaining finely aligned multimodal observations generally requires specialized coaxial sensors \cite{liao2022kitti,Silberman:ECCV12,krispel2020fuseseg} or the computation of complex mappings between each modality \cite{robert2022learning,dai20183dmv}. 
In contrast, OmniSat leverages the natural spatial alignment of EO data.  This allows us to adapt multimodal contrastive learning \cite{radford2021learning,huang2022mavil} and cross-modal masked autoencoder \cite{hackstein2024exploring} techniques to learn rich multimodal EO representations with a generalist fusion scheme. Furthermore, the alignment across modalities can be used to supervise the model to improve the representation of each modality when considered independently.

To address the scarcity of EO datasets with a diverse range of heterogeneous modalities, we enrich two existing benchmarks, TreeSatAI \cite{ahlswede2022treesatai} and PASTIS-R \cite{garnot2021panoptic,garnot2022multi}, with new and aligned modalities. This allows us to evaluate OmniSat's ability to handle an arbitrary number of inputs with varying natures and resolutions.
Our contributions can be summarized as follows.
\begin{itemize}
    \item We introduce OmniSat, a new model that learns to combine varied sources of EO observations in a self-supervised manner, resulting in richer joint representations that capture the unique characteristics of each modality.
    \item We augment two EO benchmarks to create the first datasets with three modalities of different natures, enabling future research in multimodal EO data fusion.
    \item We demonstrate that utilizing diverse modalities with a flexible model leads to better representations, establishing new state-of-the-art for tree classification,  land cover classification, and crop semantic segmentation. Additionally, we show that self-supervised training with multiple modalities leads to better performance, even when only one modality is available during inference.
\end{itemize}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{example-image}
%     \caption{{\bf Teaser.}}
%     \label{fig:enter-label}
% \end{figure}


==> z_backup_pastis/2_related.tex <==
This section provides an overview of the fields of self-supervised and multimodal learning, emphasizing how they were adapted from computer vision to Earth observation. Lastly, we highlight the scarcity of multimodal EO datasets with diverse data types.

\paragraph{\bf Self-Supervised Learning for EO.}
This technique consists in learning expressive data representations without labels by using a pretext task. This approach has been particularly successful for natural language \cite{kenton2019bert} and image \cite{oquab2023dinov2} analysis.  
Initially focused on discriminative tasks \cite{gidaris2018unsupervised,noroozi2016unsupervised,zhang2016colorful}, recent self-supervised approaches for images can be categorized either in contrastive or generative methods.

\emph{Contrastive methods} reason at the instance level and minimize the distance between representations of paired samples, often the same image under different transformations, and maximize the distance with other samples \cite{chen2020simple,he2020momentum,caron2020unsupervised}.
More efficient methods only consider positive samples and avoid mode collapse by introducing various asymmetries 
\cite{grill2020bootstrap,chen2021exploring} or normalization \cite{caron2021emerging}.
Such approaches have been successfully adapted to EO, for which samples are paired according to their location \cite{tseng2022croco} or time of acquisition \cite{ayush2021geography,manas2021seasonal}.

\emph{Generative methods} reason at the level of individual token---a small portion of the input, typically a patch for images  \cite{dosovitskiy2020image}. The objective is to reconstruct the masked tokens of an input image in pixel-space \cite{he2022masked,bao2021beit,xie2022simmim}.
This principle has been successfully adapted to EO analysis \cite{gao2022general,cong2022satmae,yuan2022sits}, and was further extended to handle multiple spatial scales  \cite{reed2023scale},  multimodality \cite{fuller2023croma,irvin2023usat}, or hyperspectral observations \cite{ibanez2022masked,liu2022band}.

Several hybrid approaches combine the discriminative power of contrastive methods and the scalability of generative objectives for natural images \cite{oquab2023dinov2,zhou2022image} and EO data \cite{fuller2023croma}. 
Our proposed OmniSat also implements both mechanisms. A key difference with other approaches is that the alignment of EO data allows us to perform contrastive learning  \emph{at the scale of tokens}.

\begin{table}[t]
\caption{\textbf{Multimodal EO Datasets.} Publicly available Earth observation datasets with multiple modalities. S1/S2 denotes Sentinel-1 or 2. \raisebox{0.3mm}{\tiny \faStar}\small~: {modalities added in this work}.}
\label{tab:datasets}
\centering
\input{tables/datasets}
\end{table}

\paragraph{\bf Self-Supervised multimodal Learning.}
Multimodal computer vision has received a lot of interest \cite{bayoudh2022survey} thanks to the success of cross-modal pre-training \cite{radford2021learning}. Recent models can align the embeddings of heterogeneous modalities such as video and sounds \cite{huang2022mavil}, depth and images \cite{hazirbas2017fusenet}, text and image \cite{baevski2022data2vec,alayrac2022flamingo}, or multiple combinations of these modalities \cite{shukor2023unival,girdhar2023imagebind,girdhar2022omnivore,srivastava2024omnivec}.

Multimodal learning also has a long history in EO \cite{yang2021muti,li2022deep,pohl1998review} due to the large variety and complementarity of sensors \cite{ghamisi2019multisource,schmitt2016data}.
However, recent transformer-based architectures \cite{vaswani2017attention} for EO are often limited to one type of modality, be it a single image \cite{cong2022satmae,reed2023scale} or time-series \cite{tarasiou2023vits,garnot2022multi}. For example, CROMA \cite{fuller2023croma} and PRESTO \cite{tseng2023lightweight}  are specifically designed for optical and radar observations, but cannot handle very high resolution (VHR) data. USat \cite{irvin2023usat} considers images with different resolutions, but only takes a single date within a time series.
UT\&T \cite{garioud2023flair} can natively take single and multi-date observations of different modalities, but cannot be easily pre-trained in a self-supervised manner since it relies on convolutions and an ad-hoc late fusion scheme.

\begin{figure}[t]
    \centering
    \input{figures/datasets}
    \caption{{\bf Datasets.} We consider three datasets:
    FLAIR (\subref{fig:data:flair}), and two new datasets. 
     We built TreeSatAI-TS (\subref{fig:data:treesat}) by adding Sentinel-1 and 2 time-series to TreeSatAI \cite{ahlswede2022treesatai}. PASTIS-HD (\subref{fig:data:pastis}) is a version of PASTIS-R \cite{garnot2022multi} enriched with VHR satellite images. \raisebox{0.3mm}{\tiny \faStar}\small~: {modalities added in this work}.
     }
    \label{fig:data}
\end{figure}

\paragraph{\bf Multimodal EO Datasets.}
\LOIC{As reported in \tabref{tab:datasets}, many multimodal EO datasets use Sentinel-1 \cite{BAO202386} and 2 \cite{Sentinel-2-paper} data for applications ranging from land cover to forestry analysis and fire detection.  We also note that most of these datasets only contain data of one type: mono-date image or time series.}
%highlighting the need for a realistic multimodal dataset: a vast majority only contain two modalities, and almost always of the same type: mono-date image or time series. 
To our knowledge, FLAIR \cite{garioud2023flair} is the only multimodal EO dataset with both very high spatial resolution ($\leq 2$m) and high temporal resolution ($>4$ images/year).
The functional map of the World \cite{christie2018functional} integrates observations from various sensors, but most areas are only observed with one sensor.
Two other datasets contain time series and single images from multiple sources, but we were not available at the time of submission:
IARPA-SMART \cite{goldberg2023automated} is not yet publicly accessible, and Satlas \cite{bastani2023satlaspretrain} requires several months of continuous download.

To showcase how OmniSat can consume an arbitrary number of modalities with different spatial, spectral, and temporal resolutions, we propose enriching existing datasets to have more than two modalities of distinct nature.
We chose the PASTIS-R \cite{garnot2022multi} and TreeSatAI \cite{ahlswede2022treesatai} datasets as their application differs from the land cover analysis of FLAIR. See \figref{fig:data} for an illustration, and \secref{sec:exp:datasets} for more details on the dataset constitution.



%motivation of self-supervized EO model
%\cite{mai2023opportunities,lacoste2021toward}
%otivation for using dedicated architectures \cite{rolf2024mission}
%\cite{gidaris2018unsupervised,noroozi2016unsupervised}
%self-supervized for CV: SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum} and SwAV \cite{caron2020unsupervised}
%mode collapse when using only positive samples by introducing BYOL \cite{grill2020bootstrap}
%SIMSAM \cite{chen2021exploring}
%DINO normalization \cite{caron2021emerging}. 
%CV: masked: \cite{he2022masked} (MAE)
%CV: masked: \cite{bao2021beit} (beit)
%CV, masked \cite{xie2022simmim} (simim)
%semi-sup for EO \cite{rsr:iclr2020}
%EO, masked \cite{gao2022general}
%EO, masked, image \cite{cong2022satmae} (satmae)
%EO, masked, image \cite{reed2023scale} (scalemae)
%EO, masked, image \cite{fuller2023croma} (croma)
%Eo, masked, image  \cite{irvin2023usat} (usat)
%EO, masked, temp \cite{bastani2023satlaspretrain}
%EO, masked, image \cite{yuan2022sits}
%EO, masked, hyper \cite{ibanez2022masked,liu2022band}

%\paragraph{\bf multimodal Learning.}
%multimodal EO is complementary
%\cite{ghamisi2019multisource,schmitt2016data}
%CROMA \cite{fuller2023croma} can consume S1 and S2 single date
%PSE-TAE \cite{garnot2020satellite,garnot2022multi} can consume S1 and S2 time series
%ss joint multimodal representations: image-text domain \cite{li2021align,yang2022vision,li2020oscar,li2022blip}

%\paragraph{\bf multimodal Earth Observation Datasets.}

%\paragraph{\bf Self-Supervised Learning (SSL)}
%aiming to learn effective representations for downstream tasks without using training labels. Self-supervised leverages the easy accessible and unlabelled data often at the expense of high computing costs. After breakthrough in natural language processing these methods have been intensively adapted to computer vision task. 
%SSL can be divided in three main groups : the discriminative and the generative methods.
%The discriminative approach consists in learning representations that can be highly distinguished according to the different inputs.
%Among these discriminative methods, contrastive methods such as SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum} and SwAV \cite{caron2020unsupervised} consist in minimizing the distance between positive sample representations obtained from the same image having undergone various transformations, while maximizing its distance to other images. Some works have been able to avoid mode collapse when using only positive samples by introducing asymmetry \cite{grill2020bootstrap,chen2021exploring} or normalization \cite{caron2021emerging}. 

%On the other hand, the generative methods seeks to reconstruct missing or corrupted parts of the input. For instance, the model has to reconstruct color \cite{zhang2016colorful}, to solve puzzle with crop of the image \cite{noroozi2016unsupervised}, to find the correct orientation of an image \cite{gidaris2018unsupervised} or to synthesis missing patches of the image \cite{he2022masked} (up to 75\%). This last approach is named Masked Image Modelling (MIM). 

%A growing number of methods are hybrid by combining global and local information in a pipeline using both discriminative and generative losses \cite{oquab2024dinov,zhou2022image}.

% Note de Nicolas : 
% Methode contrastive / Methode generative / Methode mixte / 
% But pretraining pour transferer 

%\paragraph{\bf Cross Modal}
% =/= Multi modal , in multi modal we take several modalities to get one given output / cross modal is to take into account the relation between modalities 
% désolé j'aurai pas du fermer le commentaire de Loic

%The cross modal paradigm consists in train models with more than one modality at a time in order to learn relation between them and by synergy obtained a model that is more efficient than one trained on a single modality.
%Most of the effort to build cross-modal models have been focused on vision-language setting \cite{}, while few models have been trained with more than two modalities. 
%The Flamingo method image/video text \cite{alayrac2022flamingo}
%The UnIVAL \cite{shukor2023unival} model is composed of a unified architecture that is trained on text, image and video with an unique objective (next token prediction) and then can be fine-tuned on unseen modality (such as audio) or task leading to state of the art performances. Each modality is mapped to a common space though a lightweight modality-specific projection. % texte comme modalite pivot clairement
% usually image-text or video-text
%ImageBind \cite{girdhar2023imagebind} learns a single shared representation space by leveraging multiple types of image-paired data such as depth, thermal or egocentric video. Each modality’s embedding is aligned to image embedding leading to an emergent alignment across all of the modalities. The model can be efficiently transfer to cross-modal retrieval and text-based zero-shot tasks.


%https://arxiv.org/pdf/2212.08071.pdf : Neurips
%MAViL: MAE + contrastif sur vidéo + son traité comme images
%\cite{huang2022mavil}

%https://arxiv.org/pdf/2311.15599.pdf: encore sur arxiv 
%Big multimodal system \cite{ding2023unireplknet}
%ImageBind \cite{girdhar2023imagebind}


%https://arxiv.org/pdf/2309.16283v1.pdf
%Self-supervised Cross-view Representation with tokenwise alignment
%\cite{tu2023self}

%flamingo, different modalities sent to the same space 
%Flamingo \cite{alayrac2022flamingo}

%Omnivec \cite{srivastava2024omnivec}  

%Data2Vec : \cite{baevski2022data2vec}

%CroCo:  \cite{tseng2022croco} cross modal on EO. for retrieval

%\cite{jean2019tile2vec} treat time series as single step image


% Certaines méthodes tendent à réduire la quantité d'image utilisés : Unival 
%review for deep for EO
%\cite{zhu2017deep}
%\paragraph{\bf Self supervised for geospatial} 

%Various studies have focused on exploiting the specific characteristics of geospatial data within the self-supervised paradigm to obtain better models with less annotated data. 

%The MAE approach \cite{he2022masked}  has been applied to satellite and aerial images. 
%SatMAE \cite{cong2022satmae} adapted the MAE approach \cite{he2022masked} to Sentinel-2 time series by masking token on both temporal and spectral axis. Scale MAE \cite{reed2023scale} adapt the   positional encoding to be coherent to the spatial resolution in order to have a more robust multiscale representations for remote sensing imagery.



%Towards geospatial foundation models via continual pretraining
%\cite{Mendieta2023}

%https://arxiv.org/pdf/2304.14065.pdf: 
%presto: Multi modal MAE on sentinel data: benchmark on TreeSAT
%\cite{tseng2023lightweight}

%https://arxiv.org/pdf/2207.08051.pdf: SatMAE: Mae for time series aerial images => recontruct everything
%\cite{cong2022satmae}

%https://arxiv.org/pdf/2212.14532.pdf: 
%Scale MAE: Mae for Aerial images. Adapt pos encoding o spatial resolution
%\cite{reed2023scale}

%https://arxiv.org/abs/2401.07782
%cross-sensor masked autoencoders
%\cite{hackstein2024exploring}

%https://openaccess.thecvf.com/content_CVPR_2020/papers/Garnot_Satellite_Image_Time_Series_Classification_With_Pixel-Set_Encoders_and_Temporal_CVPR_2020_paper.pdf:
%PseTAE
%\cite{garnot2020satellite}

%https://arxiv.org/pdf/2206.13188.pdf: 
%Review of self supervised methods for RS
%\cite{wang2022self}

%https://arxiv.org/pdf/2112.07558.pdf: 
%Pastis R + tae
%\cite{garnot2022multi}

%https://arxiv.org/pdf/2312.02199.pdf: 
%USat: Same transformer for all modalities. treat each channel independantly
%\cite{irvin2023usat}
%-> multimodal fusion
%->  just monodate for the TS
%->  no cross-sensor supervision
%->  super confusing paper?

%https://arxiv.org/pdf/2305.13456.pdf:
% Still under review resize all on 224 * 224*3 Test on Treesat \cite{corley2023revisiting}

%https://d-nb.info/1269097075/34:
%TreeSAT AI paper
%\cite{ahlswede2022treesatai}

%https://openaccess.thecvf.com/content/WACV2024/papers/Greenwell_WATCH_Wide-Area_Terrestrial_Change_Hypercube_WACV_2024_paper.pdf
%Un article qui fait de la fusion de modalité avec des Transformers. J'ai l'impression qu'ils font juste un max pooling sur l'axe des modalités pour les mélanger.
%\cite{greenwell2024watch}


%DATASET: there exists very few open datasets with both SITS AND high-res aerial (just FLAIR2)

%VERY FEW MODAL THAT CAN HANDLE BOTH SITS AND HIGHRES (just AT\&T)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%https://arxiv.org/abs/2111.06377: 
%MAE paper
%\cite{he2022masked}


%imagemind = align on image
%unival = align on text


%UT&T is the only method that can handle time series and THR

%few people work on more than 2 modalities (S2/THR, text-img) 




==> z_backup_pastis/3_method.tex <==
We consider a multimodal observation $x$ and denote by $\bM$ the set of $M$ available modalities. Each observation $x^m$ is \emph{spatially} split into a set $\bT$ of $T$ spatial tokens, which are defined consistently across modalities: %$$
$x^\bM_t=\{x^m_t\}_{m\in \bM}$
corresponds to $M$ distinct views of the same area with different sensors. 
\LOIC{In total, we have $M\times T$ tokens corresponding to $M$ different modalities for $T$ different spatial areas.}

Each modality $m$ has a distinct input space $\Omega^m$ such that $x^m_t \in \Omega^m$.
Our goal is to learn multimodal token representations $f^\star_t$ that capture the content of each token $t$ across all modalities in a self-supervised fashion. To achieve this, we employ cross-modal contrastive learning (\secref{sec:contrast}) and multimodal masked encoding (\secref{sec:mae}). We then give further details on the implementation of each module in \secref{sec:implem}. The overall architecture is represented in \figref{fig:pipeline}.
%
\begin{figure}[t]
    \centering
    \input{figures/pipeline}
    \caption{{\bf OmniSat Architecture.} We illustrate OmniSat for $M=3$ modalities, each split into $T=4$ tokens. 
    The $M\times T$ input tokens $x^\bM_\bT$ are encoded independently by $M$ modality-specific encoders $\Enc^\bM$, yielding the token representations $f^\bM_\bT$. The network $\comb$ combines them into multimodal representations $f^\star_\bT$.
    The embeddings $f^\bM_\bT$ are supervised by a contrastive cross-modal objective. Some of the token embeddings are masked, and the multimodal representations $f^\star_\bT$ are decoded by modality-specific networks $\Dec^\bM$ to reconstruct their corresponding inputs in $x^\bM_\bT$.}
    \label{fig:pipeline}
\end{figure}
%--------------------------------------------------------------------
\subsection{Contrastive Objective}
%--------------------------------------------------------------------
\label{sec:contrast}
We associate each modality $m$ with a dedicated encoder $\Enc^m: \Omega^m \mapsto \mathbf{R}^d$ and denote by $f^m_t = \Enc^m(x^m_t)$ the $d$-dimensional embedding of token $t$.
We would like $f^m_t$ to capture robust and expressive features of the observation $x^m_t$ beyond appearance. To do so, we build a matching objective: tokens should have consistent embeddings \emph{across modalities}. Indeed, while each modality captures distinct characteristics of $x_t$, all encodings $f^m_t$ share the same latent variable: the actual semantic content of the area covered by $t$.

In practice, we want $f^m_t$ close to $f^n_t$ for $n\neq m$, but far from $f^n_s$ for other tokens $s\neq t$. We define the positive matches of $f^m_t$ as the encodings of the same token $f^n_t$ for the other modalities $n\neq m$. 
Our loss function $\Lcon$ is defined as such:
\begin{align}
    \Lcon = \frac1{MT}
    \sum_{(m,t) \in \bM \times \bT}
    \log 
    \left(
        \frac
        {
        \sum_{n \neq m}
            \exp(\langle f^m_t, f^n_t\rangle / \gamma)
        }
        {
        \sum_{(n,s)\in \bM\times \bT \setminus (\{m\} \times I(t))}
            \exp(\langle f^m_t, f^n_s\rangle / \gamma)
        }
    \right)~,
\end{align}
with $\gamma$ a temperature parameter,  
%$\langle \cdot,\cdot\rangle$ denoting the scalar product in $\bR^d$,
and.

 similar to the multi-positive contrastive loss MIL-NCE \cite{miech2020end}


\LOIC{
As the contrastive objective aligns multimodal representations around shared features, the representations $f^\bM_\bT$ may be encouraged to overlook the distinct attributes of their modality. We address this flaw in two ways: 
(i) contrary to the standard approach, we only set negative sample pairs \emph{within different modalities};
(ii) 
 to ensure that each encoder retains modality-specific information, we incorporate a reconstruction objective, detailed in the next section.
 }

%---------------------------------------------------------------------
\subsection{Multimodal Reconstruction Objective}
%---------------------------------------------------------------------
\label{sec:mae}
This section introduces the modality combiner network $\comb$ and its reconstruction objective.
We mask a fraction of tokens $\mask \subset \bM\times \bT$ and replace their embeddings with a learned vector $f^\text{mask} \in \bR^d$. \LOIC{The masked tokens can be different in each modality.}
All tokens are then given to the modality combining network $\comb$, which outputs $T$ multimodal embeddings $f^\star_{\bT}$:
\begin{align}
    f_\bT^\star= \comb
    \left(
    \{f^m_t\}_{(m,t) \not\in \mask}
    \cup
    \{f^\text{mask}\}_{(m,t) \in \mask}
    \right)~.
\end{align}
To encourage the embeddings $f^\star_{\bT}$ to capture information from all modalities, we build a multimodal reconstruction objective.
We equip each modality $m$ with a dedicated decoder $\Dec^m:\bR^d \mapsto \Omega^m$ and write the reconstruction loss as:
\begin{align}
    \Lmae =
    \frac1{\vert \mask \vert}
    \sum_{(m,t) \in \mask} 
    \frac1{\text{dim}(\Omega^m)}
    \left\Vert 
        \Dec^m(f^\star_t) - x^m_t
    \right\Vert^2~,
\end{align}
where $\text{dim}(\Omega^m)$ is the dimension of the input space $\Omega^m$, used for normalisation purpose. The overall loss is the sum of $\Lmae$ and $\Lcon$.% weighted by a factor $\lambda_\text{contrast}=1$.

%==========================================
\subsection{Implementation }
%==========================================
\label{sec:implem}
This section presents the tokenization process, the structure of the encoder and decoder for each modality, and the architecture of the modality combiner network. In particular, we detail the design choices specific to EO data and which leverage their unique structure \cite{rolf2024mission}.

\begin{figure*}[t]
    \centering
    \input{figures/implem}
    \caption{{\bf Module's Architecture.} (\subref{fig:implem:a}) represents the encoder and decoder of image tokens, while (\subref{fig:implem:b}) illustrates their architectures for temporal tokens with a length of $L=4$ time stamps. The modality combining module $\comb$ with $T=2$ and $M=3$ is depecited in (\subref{fig:implem:c}). \NICOLAS{Elements in orange are learned.}}
    \label{fig:enter-label}
\end{figure*}


\paragraph{\bf Multimodal Tokenization.}
All modalities $\bM$ are spatially aligned through georeferencing. We use a spatial grid to produce a set of non-overlapping tokens $\bT$ consistent across all modalities, thus ensuring that $x^\bM_t$ correspond to the same area. Throughout all experiments, we use a grid with cells of $10\times10$m. An image token is then characterized by a small patch: $50\times 50$ with $0.2$m per pixel, $10\times10$ with $1$m resolution, and $1\times1$ at $10$m resolution. The tokens of Sentinel observations \cite{Sentinel-2-paper}, which have a resolution of $10$m, are temporal sequences of spectral observations.

\LOIC{
Time series from Sentinel satellites may experience registration errors spanning several meters, complicating their precise alignment with high-resolution imagery. However, leveraging a temporal sequence of satellite data mitigates these errors, as the aggregation over time tends to balance out misalignments.}

\paragraph{\bf Encoder-Decoder for Images.}
Image tokens are small patches: $\Omega^\text{img}=\bR^{C \times I \times I}$ with $I$ the size of the patches and $C$ the number of channels. As shown in \figref{fig:implem:a}, we encode these inputs with a sequence of convolutions and max-pooling layers until the spatial dimension is fully collapsed. Decoding involves a symmetric sequence of convolutions and un-pooling layers. Contrary to existing masked auto-encoders, we pass the pooling indices from the encoder's max-pooling to the decoder's un-pooling in the manner of SegNet~\cite{badrinarayanan2017segnet}. This dispenses the encoder from learning the intra-token spatial configuration and allows it to focus on the radiometric information, which may be more relevant depending on the application.
Single-pixel image tokens are encoded with a Multi-Layer Perceptron (MLP).

\paragraph{\bf Encoder-Decoder for Time Series.}
Each time series is represented by $L$ sequential observations with $C$ channels:  $\Omega^\text{TS}=\bR^{C \times L}$, each associated with its time stamp.
We encode each token of the time series using a Lightweight Temporal Attention Encoder (LTAE) model  \cite{garnot2020lightweight}, an efficient network for geospatial time series processing. We decode each embedding $f^\star_t$ into a time series by repeating it $L$ times across the temporal dimension, adding a temporal encoding for each time step, and using an MLP to map the results to size $C$. See \figref{fig:implem:b} for an illustration.

Optical time series are notoriously affected by clouds \cite{sudmanns2019assessing}. This may affect the validity of the reconstruction task: the decoder cannot know which observations are cloudy, making the reconstruction objective unpredictable. To circumvent this issue, we use the temporal attention maps of the encoder's LTAE to select dates to reconstruct: cloudless observations are more informative and should have a higher attention score \cite{russwurm2020self}. We only consider in the reconstruction loss $\Lmae$ the top $25\%$ inputs in terms of the LTAE's attention maps.

\paragraph{\bf Modality Combining Network.} 
The modality combining network $\comb$, represented in \figref{fig:implem:c}, takes $M \times T$ tokens embeddings ${f}^\bM_\bT$, some of whom can potentially be masked. 
We equip each token in $\cT$ with a Euclidean \cite{wu2021rethinking} relative positional encoding  $\{r(s,t) \mid (s,t)\in \bT^2\}$. As most EO data are captured from above (satellite or aerial), their distribution is invariant by horizontal translation, making this choice of encoding preferable to an absolute position encoding.

The modality combining module $\comb$ starts with a series of $B$ residual self-attention blocks connecting all tokens across modality and localization. We then perform cross-attention between the resulting token embeddings $g^\bM_\bT \in \bR^{d \times M \times T}$ and $T$ copies $f^\text{comb}_\bT$ of a modality combining token $f^\text{comb} \in \bR^d$ learned as a free parameter. Each copy $f^\text{comb}_t$ characterizes a given token $t$ and is spatially aligned with all tokens indexed by $t$ for the relative positional encoding $r$. The mechanism of $\comb$ writes:
\begin{align}
    g^\bM_\bT & = \text{self-attention}
    \left(
    {f}^{\bM}_{\bT}; r\right) \\
    {f}^\star_\bT & =  \text{cross-attention}
    \left(
    g^\bM_\bT, f^\text{comb}_\bT;r
    \right)~.
\end{align}

\paragraph{\bf Hyperparameters.} Throughout all experiments, we use the same configuration for OmniSat. The embedding size is $d=256$. The number of parameters in the encoders and decoders are $3.6$M and $1.8$M for the VHR images, $403$K and $96$K for optical time series, and $402$K and $95$K for radar time series. The modality combiner module is composed of $6$ residual self-attention blocks and a single cross-attention block, for a total of $3.6$M parameters. We train our model with the ADAM optimizer \cite{kingma2014adam}, with a learning rate of $10^{-4}$ for pertaining and $2\times 10^{-5}$ for fine-tuning, and a ReduceLROnPlateau scheduler \cite{reduce} with a patience of $10$ epochs and a decay rate of $0.1$. When re-implementing competing methods, we use the hyper-parameters given on their open-source repository.

%We Split the image into 16 sub images for PASTIS-R due to memory issues

==> z_backup_pastis/4_experiments.tex <==
In this section, we demonstrate OmniSat's performance across three multimodal datasets, including the two datasets introduced in this work presented in  \secref{sec:exp:datasets}. We outline our experimental protocol and our adaptation of competing methods in \secref{sec:exp:baselines}. We then present in \secref{sec:exp:exp} quantitative results and their analysis. Lastly, we conduct an ablation study to quantify the impact of each design decision in \secref{sec:exp:ablation}.
%-------------------------------------------
\subsection{Datasets}
%-------------------------------------------
\label{sec:exp:datasets}

We evaluate OmniSat on three multimodal datasets: TreeSatAI \cite{ahlswede2022treesatai}, PASTIS-R \cite{garnot2022multi}, and FLAIR \cite{garioud2023flair}.  To highlight the benefits of leveraging an arbitrary number of modalities with varying natures, we augment TreeSatAI, and PASTIS-R with additional modalities. The resulting datasets, TreeSatAI-TS and PASTIS-HD are open-access and available on this paper repository. See \figref{fig:data} for an illustration of these three datasets.

\paragraph{\bf \bf{TreeSatAI-TS}:} 
TreeSatAI \cite{ahlswede2022treesatai} is a multimodal dataset for tree species identification, containing $50,381$ patches of $60\times60$m with multi-label annotations for $20$ classes. Each patch is associated with a very high resolution RGB and near-infrared (NIR) image ($0.2$m pixel resolution), a single Sentinel-2 multi-spectral image (10m per pixel resolution, 10 bands), and a single Sentinel-1 radar image (10m per pixel resolution, 3 bands: two polarization channels and their ratio).

\LOIC{Recognizing the importance of temporal dynamics for characterizing the phenology of trees \cite{vrieling2018vegetation},} we introduce TreeSatAI-TS. This extended version leverages open-source data to add a year-long time series for each patch for both Sentinel-1 and Sentinel-2. Note that due to the weather patterns and position of the area of interest with respect to Sentinel-2's orbit, the optical time series is particularly irregular and occluded, with up to $50\%$ of acquisitions being non-exploitable. Nonetheless, we added the raw observation without pre-processing, while TreeSatAI's single dates have been manually selected.


\paragraph{\bf \textbf{PASTIS-HD}:}
The PASTIS dataset \cite{garnot2021panoptic},
is designed for semantic and panoptic segmentation of agricultural parcels using Sentinel-2 time series and covers $18$ crop types across $2433$ image time series with dimensions of $1280\times1280$m.
Each series contains between $38$ and $61$ observations with $10$ spectral bands. PASTIS-R \cite{garnot2022multi} adds the corresponding Sentinel-1 radar time series, for a total of 169,587 radar images with three bands.

To enhance the spatial resolution and utility of PASTIS, we introduce PASTIS-HD, which integrates contemporaneous VHR satellite images (SPOT 6-7 \cite{spot}), resampled to a $1$m resolution and converted to 8 bits. This enhancement significantly improves the dataset's spatial content, providing more granular information for agricultural parcel segmentation.

\paragraph{\bf FLAIR.} 
The FLAIR dataset \cite{garioud2023flair} is, to our knowledge, the only available dataset combining VHRaerial images with time series data. It comprises $77,762$ aerial images ($512\times512$ pixels, $20$cm resolution) with five channels (RGB, near-infrared and a normalized digital surface model), alongside corresponding Sentinel-2 time series ($10$m resolution, $10$ spectral bands, $20$ to $114$ observations per year). 

We follow the protocol of Irvin \etal  \cite{irvin2023usat} to convert the semantic annotations into a multi-label classification task: each patch is associated with the labels of all its pixels. This conversion allows us to evaluate all methods in the same setting and configuration as TreeSatAI.

\begin{table}[t]
    \centering
\caption{{\bf Performance on TreeSatAI-TS.} 
We report the macro-averaged F1 for multi-label tree species prediction on TreeSatAI and our extended TreeSatAI-TS dataset when fine-tuning with $10\%$ and $100\%$ of training labels.
We distinguish methods that are \textbf{best for one modality} within a dataset, \textbf{\underline{best in a dataset}} across all modalities with 10\% or 100\% labels, and the \textbf{\fbox{best overall}}~performance. $^\star$: late feature fusion with a ResNet. $\protect\Dag$: model evaluated on this dataset for the first time.}
\label{tab:tsai}
\input{tables/treesat}
\end{table}
%\if 1 0
%-------------------------------------------
\subsection{Experimental Setting}
%-------------------------------------------
\label{sec:exp:baselines}
This section details our experimental protocol and how we adapted existing algorithms to our new datasets.

%We adapt the UT\&T model \cite{garioud2023flair} to apply it to the specific datasets described above. For the two datasets with S1 time series, we add an extra UTAE branch for this extra modality that is identical to the S2 one. This branch is supervised in the similar way and it is used to produce an embedding injected into the very high resolution UNet branch. In the case of the multi-classes classification task (for TreeSatAI-TS and FLAIR), we map the segmentation prediction of each branch to the classification output with a spatial mean and followed by a learnable linear layer per modality.
%In the case of PASTIS-HD, the very high resolution segmentation prediction is reshaped with a spatial average pooling to the size of the ground truth labels.

%\paragraph{\bf }

%\cite{tseng2021cropharvest,garioud2023flair} example of averaging S2 per month
%\fi

\paragraph{\bf Evaluation Protocol.} All experiments follow a similar setting:
\begin{itemize}
    \item {\bf Pre-training (optional).} Methods that support self-supervised pre-training (OmniSat, SatMAE \cite{cong2022satmae}, ScaleMAE \cite{reed2023scale}, CROMA \cite{fuller2023croma}) are pre-trained for up to $250$ epochs on the entire training set without access to labels.
    \item {\bf Fully Supervised Fine-Tuning.} We train the resulting models using all the labels in the training set. 
    \item {\bf Semi-Supervised Fine-Tuning.} A portion ($10$ or $20\%$) of the training set, stratified by the distribution of classes, is used to fine-tune the models. This corresponds to full supervision in the low-data regime for models without pre-training.
    \item {\bf Monomodal and multimodal.} We evaluate respectively all methods using only one of the available modalities, and  by combining all supported modalities. 
\end{itemize}

\paragraph{\bf Adapting Baselines.} 
\LOIC{We report the performance of several methods taken which have been evaluated on the base datasets TreeSatAI and PASTIS: LightGBM \cite{ahlswede2022treesatai}, PRESTO \cite{tseng2023lightweight}, MOSAIKS \cite{rolf2021generalizable}, UTAE \cite{garnot2021panoptic,garnot2022multi} and TSViT \cite{tarasiou2023vits}. 
However, few existing methods can operate on single- and multi-date data at the same time.} To ensure a fair evaluation of competing approaches, we modify various state-of-the-art models to handle this combination of modalities. We performed multiple tests for each approach and kept the configurations leading to their highest performance.
\begin{itemize}
    \item {\bf Multimodality.} For methods that are not natively multimodal (PSE \cite{garnot2020satellite}, ViT \cite{dosovitskiy2020image}, SatMAE, ScaleMAE),  we employ a late-fusion scheme \cite{hong2020more}: we concatenate channel-wise the embeddings learned in each modality, as suggested by Ahlswede \etal \cite{ahlswede2022treesatai}. For UT\&T \cite{garioud2023flair}, initially designed for VHR images and Sentinel-2 time series, we add a branch for Sentinel-1 integration, which is identical to the Sentinel-2 branch except for the first layer.
    \item {\bf Handling Temporal Data.} \LOIC{To evaluate image models on time series (SatMAE, ScaleMAE, CROMA), we convert image sequences to single images by concatenating for each pixel and channel 
 channel-wise the median observation for the four seasons: spring, summer, fall, and winter \cite{kussul2017deep}.} %We use a single yearly median for TreeSatAI-TS due to its highly irregular year sampling.
    \item {\bf Handling VHR Data.} 
    \LOIC{To evaluate methods designed for low-resolution images (PSE, LTAE \cite{garnot2020lightweight}) in a multimodal setting that includes VHR images, we concatenate to their final embedding the representations obtained with a ResNet network.}
    \item {\bf Scaling Models.} \LOIC{Our considered datasets are smaller than the ones used to design the largest ViT-based models, making them prone to overfitting. 
    We address this issue by selecting} a ViT-Small \cite{dosovitskiy2020image} backbone instead of a ViT-Large for SatMAE, ScaleMAE and CROMA.
    \item {\bf Multi-Class Prediction.} To evaluate ViT-based models on classification experiments, we select the embedding of the class token $\langle\texttt{CLS}\rangle$. We insert a linear layer that maps its embedding to a vector of class scores. For the UT\&T model, we compute a spatial average of the last feature map, followed by a similar linear projection.
\end{itemize}



\begin{table}[t]   
\caption{{\bf PASTIS-HD.} We report the macro-averaged IoU for crop-type semantic segmentation on the PASTIS and PASTIS-HD datasets. We distinguish methods that are \textbf{best for one modality} within a dataset, \textbf{\underline{best in a dataset}} across all modalities, and the \textbf{\fbox{best overall}}~performance. $\protect\Dag$: model evaluated on this dataset for the first time.}
    \label{tab:pastis}
    \centering
   \input{tables/pastis}
\end{table}

\begin{table}[t]  
\caption{{\bf FLAIR.} We report the macro-averaged F1-score for land cover multi-class classification on the FLAIR dataset. We distinguish methods that are \textbf{best for one modality} and \textbf{\underline{best in a dataset}}. $\protect\Dag$: model evaluated on this dataset for the first time.}
    \label{tab:flair}
    \centering
   \input{tables/flair}
\end{table}

%-----------------------------------------------------
\subsection{Numerical Experiments and Analysis}
%-------------------------------------------------------
\label{sec:exp:exp}
In this section, we assess our model's performance and efficiency compared to other approaches across the three considered datasets.

\paragraph{\bf TreeSatAI-TS.} 
\tabref{tab:tsai} presents the performance of different models on TreeSatAI (TSAI) and TreeSatAI-TS. We report several key observations:
\begin{itemize}
    \item {\bf Benefit of Time Series.} For the original TSAI with single date Sentinel-1/Sentinel-2 observations, none of the pre-training schemes significantly improve performance over simple baselines such as ResNet, PSE, or MLP, even in a semi-supervised setting. In particular, single-date S1 observations yield low performance for all methods (below $20$ F1-score), emphasizing the need to use the entire time series.
    When evaluating on TreeSatAI-TS, methods that rely on temporal attention exhibit significantly improved results, while other methods struggle to extract meaningful dynamic features from the highly occluded time series. %We were not able to meaningfully train CROMA due to the noise inherent to high occlusions.
    %
    \item {\bf Multimodality.}  OmniSat outperforms all competing methods, with or without pre-training. The performance of OmniSat and CROMA in the multimodal setting is strictly superior to the performance of each modality individually by $3.7\%$ and $5.3$\%, respectively. This demonstrates the value of learning to combine information from different sources. In contrast, the multimodal performance of methods not designed for multimodality (SatMAE, ScaleMAE, ViT) is comparable to their best modality. 
    %
    \item {\bf Cross-Modal Pre-Training.} Our pre-training scheme enhances the $100\%$-label performance of OmniSat by 0.9\% in a multimodal setting, and up to 13.2\% when performing inference with Sentinel-2 time series alone. When fine-tuning with only $10$\% of labels, this gap grows to 8.9\% and 17.5\%, respectively. These results demonstrate that our self-supervised pre-training scheme improves not only the multimodal performance but also the monomodal set-up.
\end{itemize}

\begin{figure}[t]
    \centering
    \input{figures/time_size}
        \caption{{\bf Efficiency.} Performance of different models on TreeSatAI and TreeSatAI-TS with pre-training and fine-tuning using $100\%$ of labels. The $x$-axis is the number of trainable parameters in the models, and the area of the marker is proportional to the training time, broken down in pre-training and fine-tuning when applicable. }
    \label{fig:efficiency}
\end{figure}

\paragraph{\bf Experiments on PASTIS-HD.} 
We report in \tabref{tab:pastis} the performance of various models on PASTIS and PASTIS-HD. We observe that adding VHR images improves the overall performance. OmniSat can successfully combine all modalities despite the different resolutions, leading to better results than its best modality. We also observe that our cross-modal pretraining improves OmniSat's performance in both the multimodal and single-modality setting. 
 
\paragraph{\bf FLAIR.}
We report in \tabref{tab:flair} the results on the bimodal FLAIR dataset \NICOLAS{for the multi labels classification task. ???}

\paragraph{\bf Efficiency Evaluation.} We plot in \figref{fig:efficiency} the best performance between  TreeSatAI and TreeSatAI-TS for different models according to their size and training time. OmniSat is more compact, faster to train, and performs better than all evaluated models. The combination of PSE, LTAE, and ResNet is a strong contender, outperforming significantly more complex models with generic encoding-decoding schemes.

\if 1 0
\begin{figure}
    \centering
    \input{figures/treesat_coverage}
    \caption{{\bf Impact of pre-training.}}
    \label{fig:enter-label}
\end{figure}
\fi

%----------------------------------------------------
\subsection{Ablation Study}
%----------------------------------------------------
\label{sec:exp:ablation}

In this section, we conduct several experiments to evaluate the impact and validity of our main design choices and report the results in  \tabref{tab:ablation}.

\paragraph{\bf a) Role of Loss Functions.}
When training without contrastive loss on the encoders' embeddings, we observe a small dip in performance of $0.8$\% in the fully supervised regime and a more pronounced decrease of $5.5$\% in the semi-supervised regime. This demonstrates how harmonizing the encoding across encoders facilitates their fusion. Interestingly, when implementing a naive contrastive loss that considers negative examples in the target modality, the decrease is larger than simply removing this loss ($2$\% in full supervision, $X.X$\% with $10$\% of labels). Indeed, forcing the representation of an image to be closer to a time series'  than to another image's may lead the model to discard relevant information.

We also removed the reconstruction loss, meaning that only the encoders are learned contrastively during training. This results in a loss of X\% F1-score point, illustrating the importance of pre-training the transformer $\comb$ alongside the encoders.

\paragraph{\bf b) Encoder/Decoder Architecture.}
We proposed several improvements to the standard image encoder-decoder scheme used in computer vision to accommodate the specificities of EO data. In particular, bypassing the maxpool indices from the image patch encoder to the decoder allows the learned representation to focus on characterizing the spectral signature instead of fine-grained spatial information, leading to a performance increase of $0.7$\% in the full supervision setting.

As clouds frequently obstruct optical time series, we propose an unsupervised date-filtering scheme to only reconstruct meaningful acquisitions. This approach leads to a significant improvement of $3.6$\%, showcasing the benefit of developing modality-aware approaches for EO.

\paragraph{\bf Limitations.} 
All three datasets used in our experiments are based in Europe, primarily due to the availability of open-access annotations. This regional focus prevents us from evaluating our model's performance in tropical and developing countries, which have different environmental conditions and unique challenges. 
\NICOLAS{One of the major limitations of our current approach is its inability to perform very high-resolution fine grain segmentation. This constraint is inherently tied to the fact the model aligns modality with respect to the size of the token of the smaller resolution modality (i.e. Sentinel 1 and 2 for us). Furthermore, our methodology relies on the use of small decoders, which further restricts our ability to obtain finer segmentations.}
%It is also crucial to consider the potential implications of improving EO monitoring technologies. While our work aims to contribute to positive applications such as environmental monitoring, climate change mitigation, and food security, the same methods could potentially be employed for population control or as part of a surveillance state.

%\paragraph{\bf c) Impact of Multimodal pre-training.}

\begin{table}[t]   
\caption{{\bf Ablation Study.} We present the impact of several design choices on the TreeSatAI-TS dataset, measured in terms of macro-averaged F1-score.}
    \label{tab:ablation}
    \centering
   \input{tables/ablation}
\end{table}

